Spectroscopic Signatures of the Vanishing Natural Coronagraph of eta Carinae

Eta Carinae is a massive interacting binary system shrouded in a complex circumstellar environment whose evolution is the source of the long-term brightening observed during the last 80 years. An occulter, acting as a natural coronagraph, impacts observations from our perspective, but not from most other directions. Other sight-lines are visible to us through studies of the Homunculus reflection nebula. The coronagraph appears to be vanishing, decreasing the extinction towards the central star, and causing the star's secular brightening. In contrast, the Homunculus remains at an almost constant brightness. The coronagraph primarily suppresses the stellar continuum, to a lesser extent the wind lines, and not the circumstellar emission lines. This explains why the absolute values of equivalent widths (EWs) of the emission lines in our direct view are larger than those seen in reflected by the Homunculus, why the direct view absolute EWs are decreasing with time, and why lower-excitation spectral wind lines formed at larger radii (e.g. FeII 4585A) decrease in intensity at a faster pace than higher excitation lines that form closer to the star (e.g. H\delta). Our main result is that the star, despite its 10-fold brightening over two decades, is relatively stable. A vanishing coronagraph that can explain both the large flux evolution and the much weaker spectral evolution. This is contrary to suggestions that the long-term variability is intrinsic to the primary star that is still recovering from the Great Eruption with a decreasing mass-loss rate and a polar wind that is evolving at a slower pace than at the equator.

==> table_a3.tex <==
\begin{table}
	\centering									
	\caption{Equivalent widths in direct light for \ha.}
	\label{table-direct-ha}
	\begin{tabular}{cccc} 
    \hline							
HJD	&	EW \ha	&	$\sigma_{\rm{EW}}$	&	Site	\\
 & {(\AA)}&{(\AA)}&  \\
\hline
49063.609	&	$-$1009	&	48	&	ESO/FEROS	\\
49065.609	&	$-$1013	&	51	&	ESO/FEROS	\\
49066.621	&	$-$996	&	49	&	ESO/FEROS	\\
49067.605	&	$-$1005	&	50	&	ESO/FEROS	\\
49068.609	&	$-$1001	&	52	&	ESO/FEROS	\\
49069.609	&	$-$1009	&	50	&	ESO/FEROS	\\
49071.613	&	$-$1006	&	50	&	ESO/FEROS	\\
49072.613	&	$-$962	&	52	&	ESO/FEROS	\\
49073.648	&	$-$1004	&	49	&	ESO/FEROS	\\
49074.625	&	$-$998	&	49	&	ESO/FEROS	\\
49075.574	&	$-$986	&	47	&	ESO/FEROS	\\
49076.625	&	$-$1001	&	49	&	ESO/FEROS	\\
49077.590	&	$-$998	&	52	&	ESO/FEROS	\\
49078.613	&	$-$970	&	54	&	ESO/FEROS	\\
49079.605	&	$-$1004	&	50	&	ESO/FEROS	\\
49080.605	&	$-$982	&	50	&	ESO/FEROS	\\
49081.609	&	$-$1000	&	48	&	ESO/FEROS	\\
49082.609	&	$-$982	&	48	&	ESO/FEROS	\\
49083.598	&	$-$1011	&	55	&	ESO/FEROS	\\
49084.598	&	$-$994	&	49	&	ESO/FEROS	\\
49085.598	&	$-$987	&	51	&	ESO/FEROS	\\
49086.605	&	$-$976	&	45	&	ESO/FEROS	\\
49087.602	&	$-$988	&	48	&	ESO/FEROS	\\
49088.609	&	$-$990	&	43	&	ESO/FEROS	\\
49089.621	&	$-$970	&	48	&	ESO/FEROS	\\
49089.621	&	$-$970	&	48	&	ESO/FEROS	\\
49090.605	&	$-$958	&	45	&	ESO/FEROS	\\
49091.625	&	$-$924	&	41	&	ESO/FEROS	\\
49095.590	&	$-$988	&	43	&	ESO/FEROS	\\
49098.625	&	$-$979	&	45	&	ESO/FEROS	\\
49098.688	&	$-$972	&	41	&	ESO/FEROS	\\
49100.605	&	$-$962	&	45	&	ESO/FEROS	\\
49101.605	&	$-$1001	&	46	&	ESO/FEROS	\\
49102.605	&	$-$1005	&	43	&	ESO/FEROS	\\
49103.605	&	$-$981	&	41	&	ESO/FEROS	\\
49103.734	&	$-$959	&	40	&	ESO/FEROS	\\
49104.617	&	$-$1005	&	43	&	ESO/FEROS	\\
49105.605	&	$-$982	&	45	&	ESO/FEROS	\\
49106.605	&	$-$985	&	46	&	ESO/FEROS	\\
49108.602	&	$-$989	&	44	&	ESO/FEROS	\\
49109.605	&	$-$992	&	42	&	ESO/FEROS	\\
49110.684	&	$-$979	&	41	&	ESO/FEROS	\\
49110.684	&	$-$974	&	42	&	ESO/FEROS	\\
49111.684	&	$-$939	&	37	&	ESO/FEROS	\\
49112.680	&	$-$959	&	43	&	ESO/FEROS	\\
49113.578	&	$-$981	&	42	&	ESO/FEROS	\\
49114.676	&	$-$930	&	40	&	ESO/FEROS	\\
49118.563	&	$-$982	&	42	&	ESO/FEROS	\\
49120.676	&	$-$983	&	44	&	ESO/FEROS	\\
49121.551	&	$-$1004	&	46	&	ESO/FEROS	\\
49122.527	&	$-$985	&	43	&	ESO/FEROS	\\
49123.637	&	$-$957	&	45	&	ESO/FEROS	\\
49124.539	&	$-$1008	&	46	&	ESO/FEROS	\\
49125.535	&	$-$983	&	46	&	ESO/FEROS	\\
49127.617	&	$-$925	&	37	&	ESO/FEROS	\\
49128.539	&	$-$1008	&	42	&	ESO/FEROS	\\
49129.543	&	$-$959	&	38	&	ESO/FEROS	\\
49130.543	&	$-$998	&	48	&	ESO/FEROS	\\
49132.625	&	$-$984	&	43	&	ESO/FEROS	\\
49134.625	&	$-$995	&	46	&	ESO/FEROS	\\
49134.625	&	$-$995	&	46	&	ESO/FEROS	\\
49137.645	&	$-$973	&	42	&	ESO/FEROS	\\
49138.590	&	$-$982	&	42	&	ESO/FEROS	\\
49395.867	&	$-$1025	&	31	&	ESO/FEROS	\\
49408.532	&	$-$975	&	40	&	ESO/FEROS	\\
49424.523	&	$-$994	&	29	&	ESO/FEROS	\\
49448.605	&	$-$1046	&	24	&	ESO/FEROS	\\
49467.564	&	$-$884	&	28	&	ESO/FEROS	\\
49472.599	&	$-$905	&	22	&	ESO/FEROS	\\
49514.541	&	$-$890	&	24	&	ESO/FEROS	\\
49520.612	&	$-$878	&	24	&	ESO/FEROS	\\
49522.539	&	$-$934	&	20	&	ESO/FEROS	\\
49525.528	&	$-$867	&	31	&	ESO/FEROS	\\
49527.526	&	$-$876	&	19	&	ESO/FEROS	\\
49532.520	&	$-$905	&	20	&	ESO/FEROS	\\
49534.504	&	$-$935	&	20	&	ESO/FEROS	\\
49751.720	&	$-$1084	&	28	&	ESO/FEROS	\\
49770.738	&	$-$1156	&	28	&	ESO/FEROS	\\
49786.616	&	$-$1146	&	28	&	ESO/FEROS	\\
49800.743	&	$-$1147	&	25	&	ESO/FEROS	\\
49821.735	&	$-$1120	&	25	&	ESO/FEROS	\\
49836.552	&	$-$1176	&	29	&	ESO/FEROS	\\
49846.541	&	$-$1163	&	31	&	ESO/FEROS	\\
49860.569	&	$-$1131	&	23	&	ESO/FEROS	\\
50120.783	&	$-$1058	&	22	&	ESO/FEROS	\\
50134.773	&	$-$1144	&	22	&	ESO/FEROS	\\
50146.869	&	$-$1107	&	17	&	ESO/FEROS	\\
50160.749	&	$-$1163	&	25	&	ESO/FEROS	\\
50174.758	&	$-$1184	&	25	&	ESO/FEROS	\\
50188.813	&	$-$1043	&	23	&	ESO/FEROS	\\
50201.733	&	$-$1103	&	19	&	ESO/FEROS	\\
50238.467	&	$-$988	&	24	&	ESO/FEROS	\\
50238.484	&	$-$888	&	28	&	ESO/FEROS	\\
50238.513	&	$-$1159	&	22	&	ESO/FEROS	\\
50242.454	&	$-$1150	&	29	&	ESO/FEROS	\\
50242.471	&	$-$1160	&	26	&	ESO/FEROS	\\
50242.487	&	$-$1169	&	23	&	ESO/FEROS	\\
50244.563	&	$-$1074	&	25	&	ESO/FEROS	\\
50244.581	&	$-$1085	&	24	&	ESO/FEROS	\\
50244.598	&	$-$1079	&	25	&	ESO/FEROS	\\
50449.736	&	$-$1043	&	39	&	ESO/FEROS	\\
50449.736	&	$-$1013	&	35	&	ESO/FEROS	\\
50449.757	&	$-$987	&	35	&	ESO/FEROS	\\
50450.757	&	$-$1098	&	32	&	ESO/FEROS	\\
50450.772	&	$-$1117	&	38	&	ESO/FEROS	\\
50450.787	&	$-$1096	&	37	&	ESO/FEROS	\\
50451.692	&	$-$1109	&	40	&	ESO/FEROS	\\
50451.706	&	$-$1102	&	34	&	ESO/FEROS	\\
50451.720	&	$-$1119	&	26	&	ESO/FEROS	\\
50452.691	&	$-$1077	&	27	&	ESO/FEROS	\\
50452.705	&	$-$1068	&	44	&	ESO/FEROS	\\
50452.719	&	$-$1071	&	32	&	ESO/FEROS	\\
50453.692	&	$-$1118	&	37	&	ESO/FEROS	\\
50453.705	&	$-$1098	&	35	&	ESO/FEROS	\\
50453.719	&	$-$1136	&	30	&	ESO/FEROS	\\
50454.705	&	$-$1127	&	39	&	ESO/FEROS	\\
50454.719	&	$-$1095	&	40	&	ESO/FEROS	\\
50454.733	&	$-$1138	&	35	&	ESO/FEROS	\\
50455.798	&	$-$1092	&	28	&	ESO/FEROS	\\
50455.811	&	$-$1100	&	30	&	ESO/FEROS	\\
50455.825	&	$-$1056	&	42	&	ESO/FEROS	\\
50456.705	&	$-$1122	&	34	&	ESO/FEROS	\\
50456.719	&	$-$1130	&	32	&	ESO/FEROS	\\
50456.733	&	$-$1094	&	30	&	ESO/FEROS	\\
50457.676	&	$-$1051	&	36	&	ESO/FEROS	\\
50457.690	&	$-$1099	&	30	&	ESO/FEROS	\\
50457.703	&	$-$1115	&	30	&	ESO/FEROS	\\
50464.836	&	$-$1126	&	34	&	ESO/FEROS	\\
50464.848	&	$-$1085	&	26	&	ESO/FEROS	\\
50464.857	&	$-$1098	&	29	&	ESO/FEROS	\\
50464.867	&	$-$1099	&	29	&	ESO/FEROS	\\
50472.854	&	$-$1128	&	29	&	ESO/FEROS	\\
50472.866	&	$-$1154	&	33	&	ESO/FEROS	\\
50472.876	&	$-$1168	&	31	&	ESO/FEROS	\\
50472.886	&	$-$1181	&	33	&	ESO/FEROS	\\
50476.826	&	$-$1142	&	38	&	ESO/FEROS	\\
50476.839	&	$-$1133	&	32	&	ESO/FEROS	\\
50476.851	&	$-$1096	&	35	&	ESO/FEROS	\\
50476.864	&	$-$1144	&	32	&	ESO/FEROS	\\
50516.666	&	$-$1022	&	28	&	ESO/FEROS	\\
50516.677	&	$-$1029	&	25	&	ESO/FEROS	\\
50516.687	&	$-$1015	&	45	&	ESO/FEROS	\\
50518.615	&	$-$1049	&	23	&	ESO/FEROS	\\
50518.624	&	$-$1056	&	34	&	ESO/FEROS	\\
50518.633	&	$-$1021	&	31	&	ESO/FEROS	\\
50520.634	&	$-$900	&	31	&	ESO/FEROS	\\
50520.655	&	$-$1071	&	22	&	ESO/FEROS	\\
50522.679	&	$-$1086	&	35	&	ESO/FEROS	\\
50522.689	&	$-$1104	&	35	&	ESO/FEROS	\\
50522.698	&	$-$1074	&	32	&	ESO/FEROS	\\
50524.685	&	$-$1026	&	28	&	ESO/FEROS	\\
50524.696	&	$-$1142	&	41	&	ESO/FEROS	\\
50524.706	&	$-$1172	&	33	&	ESO/FEROS	\\
50527.619	&	$-$1019	&	30	&	ESO/FEROS	\\
50527.629	&	$-$1099	&	33	&	ESO/FEROS	\\
50527.640	&	$-$1087	&	39	&	ESO/FEROS	\\
50531.638	&	$-$993	&	28	&	ESO/FEROS	\\
50531.649	&	$-$1006	&	29	&	ESO/FEROS	\\
50531.659	&	$-$1055	&	28	&	ESO/FEROS	\\
50533.615	&	$-$1066	&	34	&	ESO/FEROS	\\
50533.625	&	$-$1018	&	29	&	ESO/FEROS	\\
50533.635	&	$-$1027	&	33	&	ESO/FEROS	\\
50535.669	&	$-$1038	&	24	&	ESO/FEROS	\\
50535.679	&	$-$1037	&	20	&	ESO/FEROS	\\
50535.689	&	$-$1042	&	25	&	ESO/FEROS	\\
50537.651	&	$-$1025	&	30	&	ESO/FEROS	\\
50537.661	&	$-$1013	&	25	&	ESO/FEROS	\\
50537.671	&	$-$1050	&	26	&	ESO/FEROS	\\
50539.650	&	$-$1026	&	22	&	ESO/FEROS	\\
50539.660	&	$-$1036	&	36	&	ESO/FEROS	\\
50539.670	&	$-$1048	&	32	&	ESO/FEROS	\\
50541.650	&	$-$1064	&	25	&	ESO/FEROS	\\
50541.660	&	$-$1064	&	33	&	ESO/FEROS	\\
50541.670	&	$-$1063	&	19	&	ESO/FEROS	\\
50543.652	&	$-$1043	&	26	&	ESO/FEROS	\\
50543.662	&	$-$1050	&	26	&	ESO/FEROS	\\
50543.672	&	$-$1044	&	24	&	ESO/FEROS	\\
50545.644	&	$-$997	&	32	&	ESO/FEROS	\\
50545.654	&	$-$1035	&	24	&	ESO/FEROS	\\
50545.664	&	$-$1028	&	23	&	ESO/FEROS	\\
50547.646	&	$-$1051	&	36	&	ESO/FEROS	\\
50547.656	&	$-$1060	&	20	&	ESO/FEROS	\\
50547.666	&	$-$1075	&	34	&	ESO/FEROS	\\
50549.648	&	$-$1078	&	22	&	ESO/FEROS	\\
50549.658	&	$-$1077	&	24	&	ESO/FEROS	\\
50549.668	&	$-$1047	&	31	&	ESO/FEROS	\\
50551.663	&	$-$1036	&	33	&	ESO/FEROS	\\
50551.673	&	$-$998	&	34	&	ESO/FEROS	\\
50551.683	&	$-$1080	&	24	&	ESO/FEROS	\\
50553.665	&	$-$1034	&	24	&	ESO/FEROS	\\
50553.675	&	$-$1031	&	34	&	ESO/FEROS	\\
50553.685	&	$-$1071	&	22	&	ESO/FEROS	\\
50556.579	&	$-$1074	&	26	&	ESO/FEROS	\\
50556.582	&	$-$1059	&	32	&	ESO/FEROS	\\
50557.603	&	$-$1163	&	36	&	ESO/FEROS	\\
50557.605	&	$-$1155	&	39	&	ESO/FEROS	\\
50557.607	&	$-$1165	&	33	&	ESO/FEROS	\\
50559.578	&	$-$1169	&	40	&	ESO/FEROS	\\
50559.579	&	$-$1127	&	40	&	ESO/FEROS	\\
50559.582	&	$-$1159	&	39	&	ESO/FEROS	\\
50561.575	&	$-$1172	&	31	&	ESO/FEROS	\\
50561.576	&	$-$1176	&	26	&	ESO/FEROS	\\
50561.578	&	$-$1167	&	34	&	ESO/FEROS	\\
50563.581	&	$-$1108	&	44	&	ESO/FEROS	\\
50563.584	&	$-$1163	&	30	&	ESO/FEROS	\\
50563.586	&	$-$1170	&	29	&	ESO/FEROS	\\
50565.574	&	$-$1123	&	34	&	ESO/FEROS	\\
50565.575	&	$-$1143	&	30	&	ESO/FEROS	\\
50565.577	&	$-$1136	&	31	&	ESO/FEROS	\\
51131.815	&	$-$870	&	55	&	ESO/FEROS	\\
51131.823	&	$-$888	&	34	&	ESO/FEROS	\\
51135.819	&	$-$835	&	37	&	ESO/FEROS	\\
51135.822	&	$-$918	&	36	&	ESO/FEROS	\\
51135.825	&	$-$919	&	36	&	ESO/FEROS	\\
51142.820	&	$-$901	&	37	&	ESO/FEROS	\\
51142.820	&	$-$884	&	40	&	ESO/FEROS	\\
51142.823	&	$-$904	&	35	&	ESO/FEROS	\\
51148.820	&	$-$916	&	60	&	ESO/FEROS	\\
51148.823	&	$-$938	&	58	&	ESO/FEROS	\\
51150.845	&	$-$822	&	58	&	ESO/FEROS	\\
51150.848	&	$-$806	&	55	&	ESO/FEROS	\\
51153.861	&	$-$805	&	88	&	ESO/FEROS	\\
51153.864	&	$-$869	&	80	&	ESO/FEROS	\\
51153.867	&	$-$839	&	88	&	ESO/FEROS	\\
51153.870	&	$-$896	&	81	&	ESO/FEROS	\\
51153.873	&	$-$871	&	77	&	ESO/FEROS	\\
51153.876	&	$-$892	&	79	&	ESO/FEROS	\\
51154.868	&	$-$899	&	67	&	ESO/FEROS	\\
51155.872	&	$-$912	&	61	&	ESO/FEROS	\\
51156.880	&	$-$900	&	63	&	ESO/FEROS	\\
51173.725	&	$-$868	&	54	&	ESO/FEROS	\\
51175.826	&	$-$926	&	65	&	ESO/FEROS	\\
51178.869	&	$-$857	&	43	&	ESO/FEROS	\\
51181.881	&	$-$873	&	44	&	ESO/FEROS	\\
51183.883	&	$-$852	&	42	&	ESO/FEROS	\\
51187.884	&	$-$852	&	45	&	ESO/FEROS	\\
51196.896	&	$-$858	&	67	&	ESO/FEROS	\\
51247.681	&	$-$894	&	41	&	ESO/FEROS	\\
51247.714	&	$-$855	&	43	&	ESO/FEROS	\\
51247.721	&	$-$1121	&	100	&	ESO/FEROS	\\
51291.574	&	$-$868	&	45	&	ESO/FEROS	\\
51291.591	&	$-$934	&	110	&	ESO/FEROS	\\
51373.459	&	$-$858	&	44	&	ESO/FEROS	\\
51374.481	&	$-$872	&	43	&	ESO/FEROS	\\
51375.448	&	$-$867	&	39	&	ESO/FEROS	\\
51376.477	&	$-$871	&	38	&	ESO/FEROS	\\
51379.459	&	$-$872	&	38	&	ESO/FEROS	\\
51380.497	&	$-$859	&	41	&	ESO/FEROS	\\
51381.485	&	$-$867	&	38	&	ESO/FEROS	\\
51382.476	&	$-$864	&	29	&	ESO/FEROS	\\
51383.466	&	$-$867	&	29	&	ESO/FEROS	\\
51384.457	&	$-$875	&	30	&	ESO/FEROS	\\
51385.479	&	$-$885	&	35	&	ESO/FEROS	\\
51386.459	&	$-$859	&	39	&	ESO/FEROS	\\
51387.502	&	$-$822	&	67	&	ESO/FEROS	\\
51388.462	&	$-$822	&	49	&	ESO/FEROS	\\
51389.457	&	$-$835	&	52	&	ESO/FEROS	\\
51390.461	&	$-$825	&	46	&	ESO/FEROS	\\
51391.496	&	$-$835	&	40	&	ESO/FEROS	\\
51392.470	&	$-$839	&	37	&	ESO/FEROS	\\
51393.483	&	$-$878	&	39	&	ESO/FEROS	\\
51394.471	&	$-$879	&	37	&	ESO/FEROS	\\
51530.799	&	$-$814	&	162	&	ESO/FEROS	\\
51530.799	&	$-$814	&	162	&	ESO/FEROS	\\
51530.802	&	$-$805	&	191	&	ESO/FEROS	\\
51532.852	&	$-$825	&	65	&	ESO/FEROS	\\
51594.910	&	$-$865	&	41	&	ESO/FEROS	\\
51654.549	&	$-$897	&	27	&	ESO/FEROS	\\
51873.848	&	$-$905	&	94	&	ESO/FEROS	\\
51873.855	&	$-$910	&	100	&	ESO/FEROS	\\
51873.857	&	$-$944	&	103	&	ESO/FEROS	\\
51873.859	&	$-$946	&	107	&	ESO/FEROS	\\
51924.748	&	$-$957	&	63	&	ESO/FEROS	\\
51924.751	&	$-$966	&	59	&	ESO/FEROS	\\
51924.755	&	$-$954	&	54	&	ESO/FEROS	\\
51927.884	&	$-$1001	&	84	&	ESO/FEROS	\\
51927.887	&	$-$998	&	64	&	ESO/FEROS	\\
51927.890	&	$-$976	&	71	&	ESO/FEROS	\\
52011.458	&	$-$811	&	54	&	ESO/FEROS	\\
52011.460	&	$-$845	&	55	&	ESO/FEROS	\\
52011.463	&	$-$840	&	60	&	ESO/FEROS	\\
52011.466	&	$-$763	&	49	&	ESO/FEROS	\\
52068.393	&	$-$783	&	14	&	OPD/Coude	\\
52068.477	&	$-$766	&	14	&	OPD/Coude	\\
52076.386	&	$-$731	&	49	&	ESO/FEROS	\\
52076.394	&	$-$726	&	50	&	ESO/FEROS	\\
52076.398	&	$-$768	&	80	&	ESO/FEROS	\\
52076.400	&	$-$824	&	69	&	ESO/FEROS	\\
52301.690	&	$-$890	&	122	&	ESO/FEROS	\\
52301.694	&	$-$918	&	38	&	ESO/FEROS	\\
52615.812	&	$-$997	&	96	&	ESO/UVES	\\
52620.846	&	$-$1002	&	78	&	ESO/UVES	\\
52684.629	&	$-$1016	&	85	&	ESO/UVES	\\
53054.599	&	$-$851	&	12	&	OPD/Coude	\\
53054.605	&	$-$851	&	13	&	OPD/Coude	\\
53064.535	&	$-$732	&	15	&	OPD/Coude	\\
53193.405	&	$-$730	&	18	&	OPD/Coude	\\
53413.883	&	$-$760	&	80	&	ESO/UVES	\\
53448.636	&	$-$777	&	55	&	ESO/UVES	\\
53580.394	&	$-$781	&	8	&	OPD/Coude	\\
53719.743	&	$-$726	&	5	&	OPD/Coude	\\
53834.607	&	$-$751	&	49	&	ESO/UVES	\\
53894.516	&	$-$796	&	44	&	ESO/UVES	\\
54475.763	&	$-$866	&	51	&	ESO/UVES	\\
54513.801	&	$-$724	&	27	&	ESO/UVES	\\
54513.802	&	$-$841	&	90	&	ESO/UVES	\\
54517.717	&	$-$831	&	45	&	ESO/UVES	\\
54535.732	&	$-$824	&	69	&	ESO/UVES	\\
54535.773	&	$-$821	&	87	&	ESO/UVES	\\
54554.778	&	$-$888	&	47	&	ESO/UVES	\\
54567.513	&	$-$887	&	67	&	ESO/UVES	\\
54583.519	&	$-$846	&	42	&	ESO/UVES	\\
54599.470	&	$-$861	&	38	&	ESO/UVES	\\
54616.531	&	$-$884	&	49	&	ESO/UVES	\\
54617.597	&	$-$878	&	64	&	ESO/UVES	\\
54629.483	&	$-$863	&	42	&	ESO/UVES	\\
54656.529	&	$-$847	&	52	&	ESO/UVES	\\
55755.402	&	$-$604	&	4	&	OPD/Coude	\\
56275.819	&	$-$639	&	6	&	CTIO/Chiron	\\
56289.798	&	$-$629	&	7	&	CTIO/Chiron	\\
56361.645	&	$-$583	&	5	&	CTIO/Chiron	\\
56401.588	&	$-$598	&	5	&	CTIO/Chiron	\\
56417.590	&	$-$605	&	5	&	CTIO/Chiron	\\
56607.846	&	$-$580	&	9	&	CTIO/Chiron	\\
56612.868	&	$-$581	&	10	&	CTIO/Chiron	\\
56621.780	&	$-$571	&	14	&	ESO/UVES	\\
56638.778	&	$-$577	&	30	&	OPD/Coude	\\
56650.846	&	$-$562	&	12	&	ESO/UVES	\\
56656.704	&	$-$569	&	6	&	CTIO/Chiron	\\
56659.710	&	$-$568	&	6	&	CTIO/Chiron	\\
56664.675	&	$-$568	&	6	&	CTIO/Chiron	\\
56670.783	&	$-$553	&	6	&	CTIO/Chiron	\\
56684.699	&	$-$567	&	16	&	ESO/UVES	\\
56687.708	&	$-$579	&	7	&	CTIO/Chiron	\\
56690.691	&	$-$570	&	6	&	CTIO/Chiron	\\
56697.726	&	$-$568	&	7	&	CTIO/Chiron	\\
56710.668	&	$-$575	&	7	&	CTIO/Chiron	\\
56712.664	&	$-$592	&	16	&	ESO/UVES	\\
56712.692	&	$-$574	&	7	&	CTIO/Chiron	\\
56718.710	&	$-$573	&	7	&	CTIO/Chiron	\\
56725.569	&	$-$573	&	7	&	CTIO/Chiron	\\
56729.560	&	$-$565	&	7	&	CTIO/Chiron	\\
56732.604	&	$-$551	&	6	&	CTIO/Chiron	\\
58474.599	&	$-$569	&	11	&	OPD/Coude	\\
58556.505	&	$-$488	&	34	&	OPD/Coude	\\
58603.423	&	$-$541	&	12	&	OPD/Coude	\\
58629.489	&	$-$531	&	7	&	OPD/Coude	\\
58708.373	&	$-$568	&	10	&	OPD/Coude	\\
\hline
\end{tabular}
\end{table}

==> table_a4.tex <==

\begin{table}
	\centering									
	\caption{Equivalent widths in direct light for \ion{Fe}{ii}$\lambda$4585.}
	\label{table-direct-fe2}
	\begin{tabular}{cccc} 
    \hline							
HJD	&	EW \ion{Fe}{ii}$\lambda$4585	&	$\sigma_{\rm{EW}}$	&	Site	\\
 & {(\AA)}&{(\AA)}&  \\
\hline48844.488	&	$-$16.1	&	1.8	&	ESO/FEROS	\\
49063.609	&	$-$15.2	&	1.7	&	ESO/FEROS	\\
49067.605	&	$-$16.0	&	1.7	&	ESO/FEROS	\\
49069.609	&	$-$16.0	&	2.8	&	ESO/FEROS	\\
49071.613	&	$-$16.1	&	1.5	&	ESO/FEROS	\\
49072.613	&	$-$15.0	&	3.2	&	ESO/FEROS	\\
49073.648	&	$-$15.3	&	1.3	&	ESO/FEROS	\\
49075.574	&	$-$15.2	&	2.3	&	ESO/FEROS	\\
49076.625	&	$-$15.0	&	2.7	&	ESO/FEROS	\\
49077.590	&	$-$15.4	&	2.3	&	ESO/FEROS	\\
49078.613	&	$-$15.9	&	1.4	&	ESO/FEROS	\\
49079.605	&	$-$17.4	&	1.8	&	ESO/FEROS	\\
49080.605	&	$-$14.1	&	1.5	&	ESO/FEROS	\\
49081.609	&	$-$14.9	&	1.2	&	ESO/FEROS	\\
49082.609	&	$-$14.8	&	1.8	&	ESO/FEROS	\\
49083.598	&	$-$15.5	&	4.0	&	ESO/FEROS	\\
49084.598	&	$-$15.2	&	1.1	&	ESO/FEROS	\\
49085.598	&	$-$14.8	&	1.3	&	ESO/FEROS	\\
49086.605	&	$-$14.0	&	1.2	&	ESO/FEROS	\\
49087.602	&	$-$14.3	&	2.0	&	ESO/FEROS	\\
49088.609	&	$-$15.7	&	2.4	&	ESO/FEROS	\\
49089.621	&	$-$14.1	&	1.2	&	ESO/FEROS	\\
49091.625	&	$-$14.7	&	24.1	&	ESO/FEROS	\\
49098.625	&	$-$19.8	&	3.9	&	ESO/FEROS	\\
49098.688	&	$-$17.1	&	3.3	&	ESO/FEROS	\\
49100.605	&	$-$15.0	&	1.6	&	ESO/FEROS	\\
49101.605	&	$-$19.0	&	1.6	&	ESO/FEROS	\\
49102.605	&	$-$15.3	&	1.4	&	ESO/FEROS	\\
49103.605	&	$-$19.1	&	2.6	&	ESO/FEROS	\\
49104.617	&	$-$14.9	&	1.2	&	ESO/FEROS	\\
49105.605	&	$-$14.3	&	1.3	&	ESO/FEROS	\\
49108.602	&	$-$14.6	&	1.4	&	ESO/FEROS	\\
49109.605	&	$-$15.7	&	1.6	&	ESO/FEROS	\\
49110.684	&	$-$15.3	&	2.4	&	ESO/FEROS	\\
49110.684	&	$-$14.7	&	0.6	&	ESO/FEROS	\\
49111.684	&	$-$14.3	&	2.0	&	ESO/FEROS	\\
49113.578	&	$-$14.8	&	2.2	&	ESO/FEROS	\\
49114.676	&	$-$14.6	&	5.1	&	ESO/FEROS	\\
49118.563	&	$-$15.9	&	2.2	&	ESO/FEROS	\\
49120.676	&	$-$14.1	&	1.8	&	ESO/FEROS	\\
49121.551	&	$-$16.4	&	1.2	&	ESO/FEROS	\\
49122.527	&	$-$14.5	&	1.1	&	ESO/FEROS	\\
49123.637	&	$-$14.3	&	1.8	&	ESO/FEROS	\\
49124.539	&	$-$15.1	&	1.1	&	ESO/FEROS	\\
49125.535	&	$-$15.0	&	1.7	&	ESO/FEROS	\\
49127.617	&	$-$15.5	&	2.0	&	ESO/FEROS	\\
49128.539	&	$-$15.1	&	1.9	&	ESO/FEROS	\\
49130.543	&	$-$14.6	&	4.8	&	ESO/FEROS	\\
49132.625	&	$-$14.7	&	2.0	&	ESO/FEROS	\\
49134.625	&	$-$14.9	&	1.7	&	ESO/FEROS	\\
49134.625	&	$-$14.9	&	1.7	&	ESO/FEROS	\\
49137.645	&	$-$16.4	&	2.1	&	ESO/FEROS	\\
49138.590	&	$-$16.9	&	1.3	&	ESO/FEROS	\\
51131.815	&	$-$17.7	&	4.1	&	ESO/FEROS	\\
51131.823	&	$-$14.1	&	0.9	&	ESO/FEROS	\\
51131.826	&	$-$13.5	&	0.2	&	ESO/FEROS	\\
51135.819	&	$-$13.6	&	2.0	&	ESO/FEROS	\\
51135.822	&	$-$15.5	&	0.8	&	ESO/FEROS	\\
51135.825	&	$-$15.0	&	0.8	&	ESO/FEROS	\\
51142.820	&	$-$15.3	&	0.8	&	ESO/FEROS	\\
51142.823	&	$-$15.5	&	0.9	&	ESO/FEROS	\\
51148.820	&	$-$16.3	&	0.8	&	ESO/FEROS	\\
51148.823	&	$-$16.4	&	0.6	&	ESO/FEROS	\\
51150.845	&	$-$13.5	&	1.7	&	ESO/FEROS	\\
51150.848	&	$-$14.3	&	2.2	&	ESO/FEROS	\\
51153.870	&	$-$14.6	&	$-$20.3	&	ESO/FEROS	\\
51154.868	&	$-$16.6	&	0.8	&	ESO/FEROS	\\
51155.872	&	$-$16.4	&	0.6	&	ESO/FEROS	\\
51156.880	&	$-$16.1	&	0.7	&	ESO/FEROS	\\
51171.708	&	$-$15.5	&	2.0	&	ESO/FEROS	\\
51173.725	&	$-$16.0	&	0.5	&	ESO/FEROS	\\
51173.811	&	$-$17.9	&	12.2	&	ESO/FEROS	\\
51175.725	&	$-$14.2	&	7.7	&	ESO/FEROS	\\
51178.869	&	$-$15.5	&	0.7	&	ESO/FEROS	\\
51181.881	&	$-$16.4	&	0.6	&	ESO/FEROS	\\
51183.883	&	$-$16.1	&	0.6	&	ESO/FEROS	\\
51187.884	&	$-$16.4	&	0.8	&	ESO/FEROS	\\
51196.896	&	$-$16.9	&	0.8	&	ESO/FEROS	\\
51247.681	&	$-$14.5	&	1.1	&	ESO/FEROS	\\
51247.714	&	$-$13.9	&	1.1	&	ESO/FEROS	\\
51291.574	&	$-$14.7	&	0.7	&	ESO/FEROS	\\
51373.459	&	$-$13.9	&	0.8	&	ESO/FEROS	\\
51374.481	&	$-$14.2	&	0.9	&	ESO/FEROS	\\
51375.448	&	$-$14.2	&	0.9	&	ESO/FEROS	\\
51376.477	&	$-$14.7	&	0.9	&	ESO/FEROS	\\
51379.459	&	$-$14.8	&	0.7	&	ESO/FEROS	\\
51380.497	&	$-$14.9	&	0.6	&	ESO/FEROS	\\
51381.485	&	$-$14.1	&	1.2	&	ESO/FEROS	\\
51382.476	&	$-$15.7	&	0.7	&	ESO/FEROS	\\
51383.466	&	$-$15.2	&	0.5	&	ESO/FEROS	\\
51384.457	&	$-$15.3	&	0.5	&	ESO/FEROS	\\
51385.479	&	$-$15.5	&	0.8	&	ESO/FEROS	\\
51386.459	&	$-$15.1	&	0.7	&	ESO/FEROS	\\
51387.502	&	$-$14.0	&	3.0	&	ESO/FEROS	\\
51388.462	&	$-$13.9	&	0.8	&	ESO/FEROS	\\
51389.457	&	$-$15.0	&	0.7	&	ESO/FEROS	\\
51390.461	&	$-$15.1	&	0.6	&	ESO/FEROS	\\
51391.496	&	$-$15.1	&	0.6	&	ESO/FEROS	\\
51392.470	&	$-$15.1	&	0.4	&	ESO/FEROS	\\
51393.483	&	$-$15.3	&	0.7	&	ESO/FEROS	\\
51394.471	&	$-$14.7	&	0.9	&	ESO/FEROS	\\
51530.799	&	$-$10.7	&	7.0	&	ESO/FEROS	\\
51530.802	&	$-$10.8	&	7.5	&	ESO/FEROS	\\
51532.852	&	$-$12.5	&	0.5	&	ESO/FEROS	\\
51594.910	&	$-$12.1	&	0.7	&	ESO/FEROS	\\
51654.549	&	$-$14.4	&	0.6	&	ESO/FEROS	\\
51873.848	&	$-$13.8	&	3.0	&	ESO/FEROS	\\
51873.855	&	$-$16.2	&	17.7	&	ESO/FEROS	\\
51873.857	&	$-$14.7	&	4.6	&	ESO/FEROS	\\
51873.859	&	$-$13.9	&	3.8	&	ESO/FEROS	\\
51924.748	&	$-$14.4	&	1.3	&	ESO/FEROS	\\
51924.751	&	$-$15.0	&	1.1	&	ESO/FEROS	\\
51924.755	&	$-$14.6	&	0.7	&	ESO/FEROS	\\
51927.884	&	$-$15.7	&	1.8	&	ESO/FEROS	\\
51927.887	&	$-$16.0	&	1.8	&	ESO/FEROS	\\
51927.890	&	$-$14.7	&	2.0	&	ESO/FEROS	\\
52011.458	&	$-$12.0	&	0.5	&	ESO/FEROS	\\
52011.460	&	$-$12.9	&	0.9	&	ESO/FEROS	\\
52011.463	&	$-$13.3	&	1.3	&	ESO/FEROS	\\
52011.466	&	$-$13.1	&	0.3	&	ESO/FEROS	\\
52076.386	&	$-$10.7	&	0.6	&	ESO/FEROS	\\
52076.394	&	$-$11.2	&	0.8	&	ESO/FEROS	\\
52076.398	&	$-$11.7	&	2.7	&	ESO/FEROS	\\
52076.400	&	$-$13.4	&	1.6	&	ESO/FEROS	\\
52301.690	&	$-$16.5	&	3.8	&	ESO/FEROS	\\
52301.694	&	$-$15.8	&	0.4	&	ESO/FEROS	\\
52620.841	&	$-$14.8	&	0.3	&	ESO/UVES	\\
52684.634	&	$-$14.8	&	0.4	&	ESO/UVES	\\
52987.682	&	$-$10.6	&	0.4	&	OPD/Coude	\\
52987.686	&	$-$11.5	&	0.2	&	OPD/Coude	\\
53055.635	&	$-$15.6	&	0.5	&	ESO/UVES	\\
53413.888	&	$-$10.9	&	0.6	&	ESO/UVES	\\
53894.521	&	$-$11.9	&	0.2	&	ESO/UVES	\\
54535.776	&	$-$9.8	&	0.4	&	ESO/UVES	\\
54535.779	&	$-$9.7	&	0.3	&	ESO/UVES	\\
54567.509	&	$-$10.2	&	0.3	&	ESO/UVES	\\
54596.471	&	$-$9.3	&	0.1	&	OPD/Coude	\\
54598.387	&	$-$9.6	&	0.2	&	OPD/Coude	\\
54599.463	&	$-$9.4	&	0.3	&	ESO/UVES	\\
54601.524	&	$-$10.6	&	0.1	&	ESO/FEROS	\\
54601.528	&	$-$10.5	&	0.1	&	ESO/FEROS	\\
54616.525	&	$-$8.8	&	0.3	&	ESO/UVES	\\
54656.532	&	$-$8.8	&	0.2	&	ESO/UVES	\\
55012.500	&	$-$7.2	&	0.2	&	OPD/Coude	\\
55013.479	&	$-$6.1	&	0.3	&	ESO/UVES	\\
55018.488	&	$-$5.3	&	0.3	&	ESO/UVES	\\
55171.500	&	$-$5.5	&	0.1	&	OPD/Coude	\\
55495.500	&	$-$6.1	&	0.3	&	OPD/Coude	\\
55689.507	&	$-$5.3	&	0.2	&	SOAR/Goodman	\\
55729.539	&	$-$4.8	&	0.2	&	SOAR/Goodman	\\
55768.497	&	$-$4.7	&	0.2	&	SOAR/Goodman	\\
55856.828	&	$-$5.0	&	0.2	&	SOAR/Goodman	\\
55856.828	&	$-$5.0	&	0.2	&	SOAR/Goodman	\\
55885.500	&	$-$5.3	&	0.3	&	OPD/Coude	\\
55893.797	&	$-$4.4	&	0.1	&	SOAR/Goodman	\\
55930.772	&	$-$4.4	&	0.1	&	SOAR/Goodman	\\
55955.819	&	$-$4.4	&	0.2	&	SOAR/Goodman	\\
55982.614	&	$-$4.7	&	0.2	&	SOAR/Goodman	\\
55989.689	&	$-$4.8	&	0.4	&	CTIO/Chiron	\\
55993.752	&	$-$5.0	&	0.5	&	CTIO/Chiron	\\
56001.726	&	$-$5.2	&	0.5	&	CTIO/Chiron	\\
56001.726	&	$-$5.2	&	0.5	&	CTIO/Chiron	\\
56003.634	&	$-$4.7	&	0.2	&	SOAR/Goodman	\\
56013.686	&	$-$4.7	&	0.5	&	CTIO/Chiron	\\
56013.686	&	$-$4.7	&	0.5	&	CTIO/Chiron	\\
56020.618	&	$-$4.8	&	0.3	&	ESO/UVES	\\
56020.619	&	$-$4.7	&	0.3	&	ESO/UVES	\\
56039.528	&	$-$4.9	&	0.1	&	SOAR/Goodman	\\
56079.499	&	$-$5.7	&	0.2	&	SOAR/Goodman	\\
56116.496	&	$-$5.2	&	0.2	&	SOAR/Goodman	\\
56136.463	&	$-$4.6	&	0.2	&	SOAR/Goodman	\\
56218.500	&	$-$5.3	&	0.3	&	OPD/Coude	\\
56236.846	&	$-$5.0	&	0.5	&	CTIO/Chiron	\\
56238.870	&	$-$5.2	&	0.7	&	CTIO/Chiron	\\
56246.794	&	$-$5.0	&	0.2	&	SOAR/Goodman	\\
56248.815	&	$-$5.5	&	0.6	&	CTIO/Chiron	\\
56254.882	&	$-$5.0	&	0.5	&	CTIO/Chiron	\\
56260.783	&	$-$5.7	&	0.7	&	CTIO/Chiron	\\
56275.819	&	$-$5.9	&	0.5	&	CTIO/Chiron	\\
56278.812	&	$-$5.4	&	0.2	&	SOAR/Goodman	\\
56289.798	&	$-$6.0	&	0.4	&	CTIO/Chiron	\\
56346.697	&	$-$5.0	&	0.1	&	SOAR/Goodman	\\
56361.581	&	$-$5.2	&	0.2	&	SOAR/Goodman	\\
56361.645	&	$-$5.2	&	0.4	&	CTIO/Chiron	\\
56401.588	&	$-$5.0	&	0.4	&	CTIO/Chiron	\\
56417.590	&	$-$5.0	&	0.5	&	CTIO/Chiron	\\
56428.484	&	$-$5.2	&	0.1	&	SOAR/Goodman	\\
56452.527	&	$-$5.7	&	0.6	&	SOAR/Goodman	\\
56488.476	&	$-$5.1	&	0.2	&	SOAR/Goodman	\\
56538.500	&	$-$5.4	&	0.3	&	OPD/Coude	\\
56607.846	&	$-$4.3	&	0.6	&	CTIO/Chiron	\\
56612.868	&	$-$4.1	&	0.5	&	CTIO/Chiron	\\
56613.836	&	$-$4.1	&	0.1	&	SOAR/Goodman	\\
56655.763	&	$-$5.0	&	0.1	&	SOAR/Goodman	\\
56656.704	&	$-$4.3	&	0.3	&	CTIO/Chiron	\\
56659.710	&	$-$4.5	&	0.4	&	CTIO/Chiron	\\
56664.675	&	$-$4.0	&	0.5	&	CTIO/Chiron	\\
56670.783	&	$-$4.4	&	0.5	&	CTIO/Chiron	\\
56672.838	&	$-$4.2	&	0.4	&	CTIO/Chiron	\\
56677.759	&	$-$4.4	&	0.5	&	CTIO/Chiron	\\
56687.708	&	$-$4.8	&	0.4	&	CTIO/Chiron	\\
56690.691	&	$-$4.9	&	0.4	&	CTIO/Chiron	\\
56697.726	&	$-$4.8	&	0.4	&	CTIO/Chiron	\\
56701.745	&	$-$4.3	&	0.4	&	OPD/Coude	\\
56705.500	&	$-$5.4	&	0.3	&	OPD/Coude	\\
56710.668	&	$-$4.4	&	0.4	&	CTIO/Chiron	\\
56712.670	&	$-$4.4	&	0.3	&	ESO/UVES	\\
56712.692	&	$-$4.2	&	0.5	&	CTIO/Chiron	\\
56718.710	&	$-$4.4	&	0.4	&	CTIO/Chiron	\\
56725.569	&	$-$4.7	&	0.4	&	CTIO/Chiron	\\
56729.560	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
56730.606	&	$-$4.2	&	0.2	&	OPD/Coude	\\
56732.604	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
57016.797	&	$-$5.0	&	0.3	&	CTIO/Chiron	\\
57018.780	&	$-$4.9	&	0.3	&	CTIO/Chiron	\\
57021.836	&	$-$4.9	&	0.3	&	CTIO/Chiron	\\
57022.753	&	$-$5.0	&	0.3	&	CTIO/Chiron	\\
57025.828	&	$-$4.8	&	0.3	&	CTIO/Chiron	\\
57026.701	&	$-$4.8	&	0.3	&	CTIO/Chiron	\\
57030.691	&	$-$4.5	&	0.3	&	CTIO/Chiron	\\
57032.818	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
57035.724	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
57037.816	&	$-$4.5	&	0.3	&	CTIO/Chiron	\\
57038.852	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
57039.833	&	$-$4.5	&	0.3	&	CTIO/Chiron	\\
57040.712	&	$-$4.5	&	0.3	&	CTIO/Chiron	\\
57043.846	&	$-$4.7	&	0.3	&	CTIO/Chiron	\\
57046.684	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
57047.685	&	$-$4.5	&	0.3	&	CTIO/Chiron	\\
57048.810	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
57050.731	&	$-$4.6	&	0.4	&	CTIO/Chiron	\\
57051.846	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
57059.789	&	$-$4.7	&	0.3	&	CTIO/Chiron	\\
57060.661	&	$-$4.5	&	0.3	&	CTIO/Chiron	\\
57061.850	&	$-$4.7	&	0.3	&	CTIO/Chiron	\\
57062.695	&	$-$4.4	&	0.3	&	CTIO/Chiron	\\
57063.734	&	$-$4.5	&	0.3	&	CTIO/Chiron	\\
57064.774	&	$-$4.3	&	0.3	&	CTIO/Chiron	\\
57068.769	&	$-$4.3	&	0.3	&	CTIO/Chiron	\\
57070.645	&	$-$4.4	&	0.3	&	CTIO/Chiron	\\
57074.798	&	$-$4.7	&	0.4	&	CTIO/Chiron	\\
57075.698	&	$-$4.5	&	0.3	&	CTIO/Chiron	\\
57078.897	&	$-$4.7	&	0.3	&	CTIO/Chiron	\\
57083.660	&	$-$4.6	&	0.3	&	CTIO/Chiron	\\
57088.639	&	$-$4.3	&	0.3	&	CTIO/Chiron	\\
57091.590	&	$-$4.3	&	0.3	&	CTIO/Chiron	\\
57092.721	&	$-$4.4	&	0.3	&	CTIO/Chiron	\\
57093.708	&	$-$4.4	&	0.3	&	CTIO/Chiron	\\
57095.798	&	$-$4.5	&	0.5	&	CTIO/Chiron	\\
57097.694	&	$-$4.5	&	0.4	&	CTIO/Chiron	\\
57104.559	&	$-$4.2	&	0.3	&	CTIO/Chiron	\\
57115.746	&	$-$4.4	&	0.4	&	CTIO/Chiron	\\
57118.554	&	$-$4.4	&	0.4	&	CTIO/Chiron	\\
57120.536	&	$-$4.3	&	0.3	&	CTIO/Chiron	\\
57124.496	&	$-$4.2	&	0.3	&	CTIO/Chiron	\\
57125.521	&	$-$4.3	&	0.4	&	CTIO/Chiron	\\
57127.616	&	$-$4.2	&	0.3	&	CTIO/Chiron	\\
57130.541	&	$-$4.3	&	0.4	&	CTIO/Chiron	\\
57132.513	&	$-$4.1	&	0.3	&	CTIO/Chiron	\\
57134.623	&	$-$4.0	&	0.2	&	CTIO/Chiron	\\
57144.690	&	$-$4.1	&	1.3	&	CTIO/Chiron	\\
57145.624	&	$-$3.9	&	0.4	&	CTIO/Chiron	\\
57147.626	&	$-$5.0	&	1.0	&	CTIO/Chiron	\\
57150.614	&	$-$4.0	&	0.3	&	CTIO/Chiron	\\
57152.588	&	$-$4.8	&	2.4	&	CTIO/Chiron	\\
57155.572	&	$-$4.1	&	0.4	&	CTIO/Chiron	\\
57161.551	&	$-$4.4	&	0.4	&	CTIO/Chiron	\\
57164.548	&	$-$4.1	&	0.4	&	CTIO/Chiron	\\
57166.531	&	$-$4.1	&	0.3	&	CTIO/Chiron	\\
57172.519	&	$-$4.1	&	0.3	&	CTIO/Chiron	\\
57174.592	&	$-$4.6	&	0.5	&	CTIO/Chiron	\\
57177.488	&	$-$4.0	&	0.4	&	CTIO/Chiron	\\
57181.447	&	$-$4.0	&	0.3	&	CTIO/Chiron	\\
57185.502	&	$-$4.2	&	0.3	&	CTIO/Chiron	\\
57189.502	&	$-$4.2	&	0.3	&	CTIO/Chiron	\\
57191.460	&	$-$4.1	&	0.3	&	CTIO/Chiron	\\
57194.499	&	$-$4.2	&	0.3	&	CTIO/Chiron	\\
57443.957	&	$-$4.2	&	0.2	&	OPD/Coude	\\
58680.840	&	$-$4.2	&	0.2	&	OPD/Coude	\\
58729.847	&	$-$4.3	&	0.2	&	OPD/Coude	\\
\hline
\end{tabular}
\end{table}

==> table_a5.tex <==
\begin{table}
	\centering									
	\caption{Equivalent widths in direct star for \hd.}
	\label{table-direct-hd}
	\begin{tabular}{cccc} 
    \hline							
HJD	&	EW \hd	&	$\sigma_{\rm{EW}}$	&	Site	\\
 & {(\AA)}&{(\AA)}&  \\
\hline
58502.451	&	$-$27.4	&	1.0	&	LCO/NRES	\\
59039.234	&	$-$25.4	&	2.0	&	LCO/NRES	\\
59051.232	&	$-$26.4	&	0.6	&	LCO/NRES	\\
59152.602	&	$-$24.1	&	1.4	&	LCO/NRES	\\
59155.600	&	$-$25.0	&	1.2	&	LCO/NRES	\\
59174.562	&	$-$24.6	&	0.8	&	LCO/NRES	\\
59206.513	&	$-$23.8	&	1.1	&	LCO/NRES	\\
59210.463	&	$-$24.5	&	0.9	&	LCO/NRES	\\
49063.609	&	$-$28.8	&	13.5	&	ESO/FEROS	\\
49065.609	&	$-$32.5	&	12.2	&	ESO/FEROS	\\
49067.605	&	$-$30.3	&	11.7	&	ESO/FEROS	\\
49068.609	&	$-$30.1	&	29.0	&	ESO/FEROS	\\
49069.609	&	$-$31.9	&	30.2	&	ESO/FEROS	\\
49071.613	&	$-$29.7	&	12.0	&	ESO/FEROS	\\
49072.613	&	$-$32.4	&	49.3	&	ESO/FEROS	\\
49074.625	&	$-$27.6	&	10.9	&	ESO/FEROS	\\
49076.625	&	$-$25.4	&	7.9	&	ESO/FEROS	\\
49077.590	&	$-$26.3	&	14.5	&	ESO/FEROS	\\
49078.613	&	$-$26.7	&	13.7	&	ESO/FEROS	\\
49080.605	&	$-$26.8	&	12.5	&	ESO/FEROS	\\
49081.609	&	$-$32.7	&	33.6	&	ESO/FEROS	\\
49082.609	&	$-$28.3	&	14.6	&	ESO/FEROS	\\
49083.598	&	$-$31.9	&	9.7	&	ESO/FEROS	\\
49084.598	&	$-$29.9	&	11.3	&	ESO/FEROS	\\
49085.598	&	$-$31.8	&	10.4	&	ESO/FEROS	\\
49086.605	&	$-$29.0	&	11.2	&	ESO/FEROS	\\
49087.602	&	$-$31.4	&	11.6	&	ESO/FEROS	\\
49088.609	&	$-$26.9	&	9.2	&	ESO/FEROS	\\
49090.605	&	$-$27.2	&	24.0	&	ESO/FEROS	\\
49091.625	&	$-$29.9	&	16.9	&	ESO/FEROS	\\
49100.605	&	$-$26.6	&	18.1	&	ESO/FEROS	\\
49101.605	&	$-$28.1	&	9.5	&	ESO/FEROS	\\
49102.605	&	$-$24.4	&	4.1	&	ESO/FEROS	\\
49110.684	&	$-$27.6	&	14.6	&	ESO/FEROS	\\
49112.680	&	$-$28.8	&	27.7	&	ESO/FEROS	\\
49120.676	&	$-$25.7	&	16.1	&	ESO/FEROS	\\
49121.551	&	$-$28.6	&	19.5	&	ESO/FEROS	\\
49123.637	&	$-$28.9	&	18.0	&	ESO/FEROS	\\
49125.535	&	$-$26.5	&	18.1	&	ESO/FEROS	\\
49127.617	&	$-$31.2	&	17.8	&	ESO/FEROS	\\
49129.543	&	$-$28.5	&	9.9	&	ESO/FEROS	\\
49138.590	&	$-$27.0	&	10.3	&	ESO/FEROS	\\
49395.867	&	$-$27.6	&	9.7	&	ESO/FEROS	\\
49408.532	&	$-$29.6	&	6.3	&	ESO/FEROS	\\
49424.523	&	$-$30.2	&	14.5	&	ESO/FEROS	\\
49448.605	&	$-$30.9	&	16.4	&	ESO/FEROS	\\
49472.599	&	$-$27.9	&	6.0	&	ESO/FEROS	\\
49520.612	&	$-$26.2	&	5.6	&	ESO/FEROS	\\
49522.539	&	$-$25.3	&	5.0	&	ESO/FEROS	\\
49532.520	&	$-$29.7	&	8.1	&	ESO/FEROS	\\
49532.520	&	$-$29.7	&	8.2	&	OPD?Coude	\\
49534.504	&	$-$27.6	&	7.1	&	OPD?Coude	\\
49534.504	&	$-$27.6	&	7.1	&	ESO/FEROS	\\
49770.738	&	$-$28.5	&	3.8	&	ESO/FEROS	\\
49800.743	&	$-$26.5	&	5.1	&	ESO/FEROS	\\
49836.552	&	$-$32.1	&	6.0	&	ESO/FEROS	\\
49846.541	&	$-$32.1	&	14.7	&	ESO/FEROS	\\
49860.569	&	$-$32.6	&	12.5	&	ESO/FEROS	\\
50120.783	&	$-$30.7	&	9.2	&	ESO/FEROS	\\
50238.485	&	$-$28.1	&	6.7	&	ESO/FEROS	\\
50238.513	&	$-$27.9	&	5.0	&	ESO/FEROS	\\
50242.454	&	$-$30.6	&	15.9	&	ESO/FEROS	\\
50242.472	&	$-$25.0	&	5.6	&	ESO/FEROS	\\
50242.488	&	$-$30.0	&	5.5	&	ESO/FEROS	\\
50242.518	&	$-$28.7	&	2.3	&	ESO/FEROS	\\
50244.581	&	$-$25.9	&	10.7	&	ESO/FEROS	\\
50449.751	&	$-$26.4	&	4.6	&	ESO/FEROS	\\
50450.773	&	$-$28.0	&	4.0	&	ESO/FEROS	\\
50452.706	&	$-$27.2	&	4.4	&	ESO/FEROS	\\
50453.707	&	$-$28.2	&	4.4	&	ESO/FEROS	\\
50454.721	&	$-$28.2	&	4.3	&	ESO/FEROS	\\
50455.813	&	$-$28.0	&	3.7	&	ESO/FEROS	\\
50456.721	&	$-$28.2	&	3.6	&	ESO/FEROS	\\
50457.691	&	$-$28.2	&	3.8	&	ESO/FEROS	\\
50464.850	&	$-$29.6	&	3.5	&	ESO/FEROS	\\
50472.870	&	$-$29.8	&	3.6	&	ESO/FEROS	\\
50476.846	&	$-$28.3	&	3.6	&	ESO/FEROS	\\
50516.677	&	$-$26.6	&	3.9	&	ESO/FEROS	\\
50518.628	&	$-$27.1	&	3.7	&	ESO/FEROS	\\
50522.691	&	$-$27.6	&	4.4	&	ESO/FEROS	\\
50524.695	&	$-$27.4	&	4.2	&	ESO/FEROS	\\
50527.630	&	$-$27.4	&	3.3	&	ESO/FEROS	\\
50531.648	&	$-$27.1	&	3.7	&	ESO/FEROS	\\
50533.625	&	$-$26.7	&	3.9	&	ESO/FEROS	\\
50535.678	&	$-$27.1	&	3.4	&	ESO/FEROS	\\
50537.661	&	$-$27.4	&	3.4	&	ESO/FEROS	\\
50539.660	&	$-$27.2	&	3.3	&	ESO/FEROS	\\
50541.659	&	$-$27.4	&	3.4	&	ESO/FEROS	\\
50542.500	&	$-$27.8	&	3.7	&	ESO/FEROS	\\
50545.654	&	$-$27.7	&	3.3	&	ESO/FEROS	\\
50547.656	&	$-$27.5	&	3.6	&	ESO/FEROS	\\
50549.658	&	$-$28.4	&	3.2	&	ESO/FEROS	\\
50551.673	&	$-$28.1	&	3.7	&	ESO/FEROS	\\
50553.676	&	$-$28.0	&	3.8	&	ESO/FEROS	\\
50556.583	&	$-$27.6	&	4.2	&	ESO/FEROS	\\
50557.606	&	$-$29.8	&	4.1	&	ESO/FEROS	\\
50559.581	&	$-$30.2	&	9.9	&	ESO/FEROS	\\
50561.580	&	$-$31.2	&	9.7	&	ESO/FEROS	\\
50563.586	&	$-$30.3	&	9.8	&	ESO/FEROS	\\
50565.578	&	$-$30.4	&	9.8	&	ESO/FEROS	\\
51131.815	&	$-$27.4	&	6.9	&	ESO/FEROS	\\
51131.823	&	$-$26.2	&	2.0	&	ESO/FEROS	\\
51131.826	&	$-$26.3	&	1.0	&	ESO/FEROS	\\
51135.819	&	$-$25.0	&	4.1	&	ESO/FEROS	\\
51135.822	&	$-$27.2	&	2.1	&	ESO/FEROS	\\
51135.825	&	$-$27.1	&	1.9	&	ESO/FEROS	\\
51142.820	&	$-$27.7	&	3.9	&	ESO/FEROS	\\
51142.823	&	$-$27.4	&	2.2	&	ESO/FEROS	\\
51148.820	&	$-$28.7	&	1.9	&	ESO/FEROS	\\
51148.823	&	$-$28.8	&	1.9	&	ESO/FEROS	\\
51150.845	&	$-$25.1	&	2.6	&	ESO/FEROS	\\
51150.848	&	$-$24.5	&	3.4	&	ESO/FEROS	\\
51153.861	&	$-$26.7	&	10.3	&	ESO/FEROS	\\
51153.864	&	$-$26.3	&	8.5	&	ESO/FEROS	\\
51153.870	&	$-$28.4	&	6.4	&	ESO/FEROS	\\
51153.873	&	$-$27.5	&	6.5	&	ESO/FEROS	\\
51153.876	&	$-$27.3	&	6.8	&	ESO/FEROS	\\
51154.868	&	$-$28.2	&	2.2	&	ESO/FEROS	\\
51155.872	&	$-$28.7	&	1.6	&	ESO/FEROS	\\
51156.880	&	$-$26.9	&	2.3	&	ESO/FEROS	\\
51171.708	&	$-$25.0	&	3.6	&	ESO/FEROS	\\
51173.725	&	$-$27.5	&	1.3	&	ESO/FEROS	\\
51178.869	&	$-$27.2	&	1.5	&	ESO/FEROS	\\
51181.881	&	$-$27.8	&	1.5	&	ESO/FEROS	\\
51182.823	&	$-$30.0	&	23.1	&	ESO/FEROS	\\
51183.883	&	$-$30.6	&	1.7	&	ESO/FEROS	\\
51187.884	&	$-$27.3	&	1.7	&	ESO/FEROS	\\
51196.896	&	$-$29.8	&	42.5	&	ESO/FEROS	\\
51247.681	&	$-$27.3	&	2.9	&	ESO/FEROS	\\
51247.714	&	$-$26.8	&	2.7	&	ESO/FEROS	\\
51247.721	&	$-$27.4	&	2.5	&	ESO/FEROS	\\
51375.448	&	$-$29.7	&	2.7	&	ESO/FEROS	\\
51382.476	&	$-$29.1	&	2.4	&	ESO/FEROS	\\
51383.466	&	$-$25.7	&	1.6	&	ESO/FEROS	\\
51384.457	&	$-$26.0	&	1.7	&	ESO/FEROS	\\
51388.462	&	$-$27.9	&	2.4	&	ESO/FEROS	\\
51390.461	&	$-$25.4	&	1.5	&	ESO/FEROS	\\
51391.496	&	$-$24.4	&	1.9	&	ESO/FEROS	\\
51392.470	&	$-$25.7	&	1.7	&	ESO/FEROS	\\
51654.549	&	$-$28.0	&	1.8	&	ESO/FEROS	\\
51873.848	&	$-$28.7	&	8.8	&	ESO/FEROS	\\
51873.855	&	$-$30.8	&	11.0	&	ESO/FEROS	\\
51873.857	&	$-$26.6	&	13.9	&	ESO/FEROS	\\
51873.859	&	$-$27.3	&	13.2	&	ESO/FEROS	\\
51924.751	&	$-$25.4	&	2.9	&	ESO/FEROS	\\
51924.755	&	$-$28.2	&	1.7	&	ESO/FEROS	\\
52011.460	&	$-$24.7	&	2.9	&	ESO/FEROS	\\
52011.466	&	$-$27.4	&	1.2	&	ESO/FEROS	\\
52301.694	&	$-$28.8	&	1.4	&	ESO/FEROS	\\
54601.524	&	$-$30.3	&	0.7	&	ESO/FEROS	\\
54601.528	&	$-$30.6	&	0.7	&	ESO/FEROS	\\
56278.812	&	$-$25.2	&	0.4	&	SOAR/Goodman	\\
56278.812	&	$-$25.2	&	0.4	&	SOAR/Goodman	\\
52987.682	&	$-$25.2	&	4.1	&	OPD/Coude	\\
52987.686	&	$-$27.2	&	1.9	&	OPD/Coude	\\
53054.560	&	$-$27.3	&	1.1	&	OPD/Coude	\\
53582.412	&	$-$28.8	&	1.2	&	OPD/Coude	\\
52620.841	&	$-$26.5	&	1.7	&	ESO/UVES	\\
52684.634	&	$-$26.6	&	1.6	&	ESO/UVES	\\
53055.635	&	$-$27.1	&	0.6	&	ESO/UVES	\\
53413.888	&	$-$26.0	&	2.4	&	ESO/UVES	\\
53894.521	&	$-$26.8	&	2.5	&	ESO/UVES	\\
54535.776	&	$-$28.8	&	1.2	&	ESO/UVES	\\
54535.779	&	$-$28.9	&	1.0	&	ESO/UVES	\\
54567.509	&	$-$28.6	&	0.9	&	ESO/UVES	\\
54599.463	&	$-$27.3	&	1.1	&	ESO/UVES	\\
54616.525	&	$-$27.1	&	1.1	&	ESO/UVES	\\
54656.532	&	$-$25.9	&	0.8	&	ESO/UVES	\\
56020.618	&	$-$26.1	&	0.5	&	ESO/UVES	\\
56020.619	&	$-$26.3	&	0.6	&	ESO/UVES	\\
56650.841	&	$-$27.2	&	0.6	&	ESO/UVES	\\
56712.670	&	$-$27.0	&	0.6	&	ESO/UVES	\\
\hline
\end{tabular}
\end{table}
